A Formal TLS Handshake Model in LNT

Testing of network services represents one of the biggest challenges in cyber security. Because new vulnerabilities are detected on a regular basis, more research is needed. These faults have their roots in the software development cycle or because of intrinsic leaks in the system specification. Conformance testing checks whether a system behaves according to its specification. Here model-based testing provides several methods for automated detection of shortcomings. The formal specification of a system behavior represents the starting point of the testing process. In this paper, a widely used cryptographic protocol is specified and tested for conformance with a test execution framework. The first empirical results are presented and discussed.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{John P. Gallagher, Rob van Glabbeek and Wendelin Serwe (Eds):\\
Models for Formal Analysis of Real Systems (MARS'18)\\
and Verification and Program Transformation (VPT'18)
\\
EPTCS 268, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.268.1}{10.4204/EPTCS.268.1}}
\pdfoutput=1

